Chat, Shift and Perform: Bridging the Gap between Task-oriented and Non-task-oriented Dialog Systems

We propose CASPER (ChAt, Shift and PERform), a novel dialog system consisting of three types of dialog models: chatter, shifter, and performer. Shifter, which is designed for topic switching, enables a seamless flow of dialog from open-domain chat- to task-oriented dialog. In a user study, CASPER gave a better impression in terms of naturalness of response, lack of forced topic switching, and satisfaction compared with a baseline dialog system trained in an end-to-end manner. In an ablation study, we found that naturalness of response, dialog satisfaction, and task-elicitation rate improved compared with when shifter was removed from CASPER, indicating that topic shift with shifter supports the introduction of natural task-oriented dialog.

==> old_introduction.tex <==
\section{Introduction}
本研究では，自由形式対話における言語タスクの遂行を取り扱う．
近年は，スマートスピーカーの普及により対話形式で言語タスクを遂行する機会が増えてきた．
人はAIアシスタントなどの機械的なインタフェースに対して，人と同じように接する\cite{media_equation}．
したがって，型にはまった形式の対話でなくともユーザがAIアシスタントを使えることは必要である．
人の自由形式な発話に対する応答文を生成するには，予め用意した応答文形式から選択する手法\cite{crm,saur,ear,opendialkg}と，
DNNを利用した生成手法\cite{redial,cr-walker}がある．
DNNによる生成手法は，比較的少ない労力で広範囲な応答文生成が可能なため有望な手段である．しかし，適切に言語タスクを遂行するにはタスクに関連する知識にアクセスする必要がある．
Seq2seq対話システム\cite{seq2seq}は，多種のドメインに渡る教師データを学習することで汎化させることが可能だが，タスクを遂行するためには，むしろ狭いドメインにおける深い知識が必要である．
この問題に対してアプローチした研究は次のようなものがある．
1つ目に，ネットワークとデータを巨大にし，生成モデルが持つ重みが内包する知識を，タスクを遂行できるほど深くする\cite{gpt2,gpt3}というものである．2つ目に，Knowledge grounded models\cite{knowledge_grounded,knowledge_aware}がある．タスクに必要な知識を生成モデルの外部に用意し，Attentionを用いてslot-fillingなどの形式で知識を取り出す．3つ目に，対話システムとタスク遂行システムを分けて用意し，相互に補助し合うもがの\cite{kbrd,cr-walker}ある．

DNNを用いた自由形式対話の実現により，ボットとの対話体験は良くなった．
一方で，ユーザの発話がタスクのOODへ及ぶ可能性が出てきた．
選択式やyes/noで答えるような対話は，NLUを簡易にするだけでなく，
ドメインの絞り込みにも機能していたからである．

OOD発話を入力されても対話継続可能なタスク指向対話システムの実現に向けた研究は，次のようなものがある．
\cite{ner_seq2seq,knowledge_grounded,knowledge_aware}はタスク固有な情報をNLUおよびNLGの外部に移すことで，タスク用のモデルであってもオープンドメインな対話を可能にした．
\cite{chat_detection,adversarial_chat_detection}は雑談モデルとタスク指向対話モデルの使い分けに向けて，雑談かタスクか，どちらのqueryをユーザが入力したのか判別するモデルを作った．

これらの既存研究はいずれも，雑談とタスク指向対話の両者をこなせる対話システムの実現に貢献した．
しかし，実際に雑談とタスク指向対話を一つの対話内で実現することを考えると，その間の話題転換が必須となる．
雑談からタスクへの話題転換に関する検討については，既存研究は不十分である．
OODから戻らなければユーザにタスクは遂行させらないが，OODから強引に戻れば対話が破綻する．
したがって，OODへ入った時に，タスクへ誘導することが大事である．従来のシステムは，OODからタスクへの話題転換を扱ってない．
話題転換のモチベーションをシステムに与えなければ，OODを検出したとしても，システムの取れる行動は2通りである．
すなわち，対話破綻か，OODから復帰できず偶然戻るのを待つか．
対話が自由形式でありながら，システムが予め想定したドメイン内の対話でしか機能しない場合，ユーザは特別な気遣いを持ってシステムと接する必要がある．
それは，システムが対応可能な話題エリアを予測し，そこからはみ出さないように対話するという気遣いである．
これは，AIアシスタントと人間のように対話したがる多くのユーザにとって，極めて困難なことである．
特に，タスクに特別関心が無いユーザはOODから復帰する意欲がなく，対話によってタスクを遂行することは極めて困難である．

我々は，雑談対話システムと，タスク指向対話システムに追加して，話題転換を専任するトピック転換システム（topic shifter）を導入することで，オープンドメインな雑談とタスク指向対話を，話題転換込みで両立する．
自由形式かつ自由ドメインな対話の中でtopic shifterが応答することでシステムの設計したタスクへユーザを誘導した後，タスクを遂行させることができる．
これにより，ユーザがOODへ逸れた際の復帰が可能なだけでなく，タスク遂行に自発的な関心がないユーザに対しても，
文脈遷移に基づいてリーチ可能性の高いタスクを遂行させることができる．

topic shifterはオープンドメインな対話データで学習したSeq2seq (chatter)の転移学習によって，タスクが属するドメインの数だけ作る．
生成手法において発話傾向を操作する手法に，\cite{emo_hred}がある．彼らはユーザの感情がポジティブになるようなシステムの発話を集めたデータセットを構築することでデータセットにバイアスをかけて発話傾向を操作した．
我々はこれに習い，ユーザに遂行させたい任意のタスクに関して，そのタスクが属するドメインへ話題が移動した対話データを収集し，ドメイン転換地点となった発話文を教師データとして転移学習を行う．
これにより，topic shifterは自身のドメインへの話題転換をするモチベーションをもった対話システムになる．
また，複数のtopic shifterとchatterの使い分けは対話contextの遷移履歴から尤度を推定して行う．
上記で収集した話題転換データを用いて，ある対話コンテキストにおいて次のタイムステップに話題転換がなされるか否かを文書分類により求める．



